Regression modelling of spatiotemporal extreme U.S. wildfires via partially-interpretable neural networks

Risk management in many environmental settings requires an understanding of the mechanisms that drive extreme events. Useful metrics for quantifying such risk are extreme quantiles of response variables conditioned on predictor variables that describe, e.g., climate, biosphere and environmental states. Typically these quantiles lie outside the range of observable data and so, for estimation, require specification of parametric extreme value models within a regression framework. Classical approaches in this context utilise linear or additive relationships between predictor and response variables and suffer in either their predictive capabilities or computational efficiency; moreover, their simplicity is unlikely to capture the truly complex structures that lead to the creation of extreme wildfires. In this paper, we propose a new methodological framework for performing extreme quantile regression using artificial neutral networks, which are able to capture complex non-linear relationships and scale well to high-dimensional data. The "black box" nature of neural networks means that they lack the desirable trait of interpretability often favoured by practitioners; thus, we unify linear, and additive, regression methodology with deep learning to create partially-interpretable neural networks that can be used for statistical inference but retain high prediction accuracy. To complement this methodology, we further propose a novel point process model for extreme values which overcomes the finite lower-endpoint problem associated with the generalised extreme value class of distributions. Efficacy of our unified framework is illustrated on U.S. wildfire data with a high-dimensional predictor set and we illustrate vast improvements in predictive performance over linear and spline-based regression techniques.

==> macros.tex <==
% LaTeX macros

% Last modified: 24/2/2008


%----------------------------------------------
%  A. C. Davison, Institute of Mathematics,
%  EPFL, 1015 Lausanne, Switzerland
%  00 41 21 693 5502
%----------------------------------------------

% mathematical symbols, etc.

\def\half{{\textstyle{1\over 2}}}
\def\third{{\textstyle{1\over 3}}}
\def\quarter{{\textstyle{1\over 4}}}
\def\sixth{{\textstyle{1\over 6}}}
\def\frac#1#2{{\textstyle{#1\over#2}}}
\def\Beta{{\rm B}}

\def\argmin{{\rm argmin}}  
\def\diag{{\rm diag}}  
\def\mod{{\rm mod}}  
\def\tr{{\rm tr}}
\def\sign{{\rm sign}}
\def\ow{{\rm otherwise}}  
\def\obs{{\rm obs}}  
\def\endex{{\hfill{\color{red}$\bullet$}\medskip}}
\def\Endex{{\hfill{$\bullet$}\medskip}}
\def\redbf#1{{\color{red}\bf #1}}%
\def\red#1{{\color{red} #1}}%
\def\white#1{{\color{black} #1}}%

\DeclareSymbolFont{AMSb}{U}{msb}{m}{n}
\DeclareMathSymbol{\Natural}{\mathbin}{AMSb}{"4E}
\DeclareMathSymbol{\Integer}{\mathbin}{AMSb}{"5A}
\DeclareMathSymbol{\Real}{\mathbin}{AMSb}{"52}
\DeclareMathSymbol{\Rational}{\mathbin}{AMSb}{"51}
\DeclareMathSymbol{\Imaginary}{\mathbin}{AMSb}{"49}
\DeclareMathSymbol{\Complex}{\mathbin}{AMSb}{"43} 
\DeclareMathSymbol{\Disk}{\mathbin}{AMSb}{"44} 
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\bd{\begin{description}}
\def\ed{\end{description}}
\def\ben{\begin{enumerate}}
\def\een{\end{enumerate}}
\def\bv{\begin{verbatim}}
\def\ev{\end{verbatim}}

\def\bth{{$b{\rm th}$ }}
\def\cth{{$c{\rm th}$ }}
\def\dth{{$d{\rm th}$ }}
\def\fth{{$f{\rm th}$ }}
\def\gth{{$g{\rm th}$ }}
\def\hth{{$h{\rm th}$ }}
\def\ith{{$i{\rm th}$ }}
\def\jth{{$j{\rm th}$ }}
\def\kth{{$k{\rm th}$ }}
\def\lth{{$l{\rm th}$ }}
\def\mth{{$m{\rm th}$ }}
\def\nth{{$n{\rm th}$ }}
\def\pth{{$p{\rm th}$ }}
\def\rth{{$r{\rm th}$ }}
\def\sth{{$s{\rm th}$ }}
\def\tth{{$t{\rm th}$ }}
\def\uth{{$u{\rm th}$ }}
\def\vth{{$v{\rm th}$ }}
\def\wth{{$w{\rm th}$ }}

\def\calA{{\mathcal A}}
\def\calB{{\mathcal B}}
\def\calC{{\mathcal C}}
\def\calD{{\mathcal D}}
\def\calE{{\mathcal E}}
\def\F{{\mathcal F}}
\def\G{{\mathcal G}}
\def\H{{\mathcal H}}
\def\calH{{\mathcal H}}
\def\IG{{\mathcal IG}}
\def\cI{{\mathcal I}}
\def\cP{{\mathcal P}}
\def\calJ{{\mathcal J}}
\def\calL{{\mathcal L}}
\def\calK{{\mathcal K}}
\def\calM{{\mathcal M}}
\def\calN{{\mathcal N}}
\def\N{{\calN}}
\def\calP{{\mathcal{P}}}
\def\calQ{{\mathcal{Q}}}
\def\calO{{\mathcal{O}}}
\def\calS{{\mathcal{S}}}
\def\calI{{\mathcal{I}}}
\def\calR{{\mathcal R}}
\def\calT{{\mathcal T}}
\def\calU{{\mathcal U}}
\def\calV{{\mathcal V}}
\def\calW{{\mathcal W}}
\def\calX{{\mathcal X}}
\def\calY{{\mathcal Y}}
\def\calZ{{\mathcal Z}}
\def\W{{\mathcal W}}
\def\U{{\Upsilon}}
\def\f{\frac}
\def\l{{\lambda}}
\def\d{{\delta}}
\def\bX{{\bar X}}
\def\s{{\sigma}}
\def\p{{\partial}}
\def\p{{d}}
\def\v{{\varepsilon}}
\def\dis{{\displaystyle}}
\def\a{{\alpha}}
\def\b{{\beta}}
\def\hash{{\#}}
\def\bar#1{{\overline{#1}}}
\def\hat#1{{\widehat{#1}}}
\def\barY{{\overline{Y}}}
\def\barX{{\overline{X}}}
\def\barZ{{\overline{Z}}}
\def\barx{{\overline{x}}}
\def\bary{{\overline{y}}}
\def\barz{{\overline{z}}}
\def\T{{ \mathrm{\scriptscriptstyle T} }}
\def\mT{{ -\mathrm{\scriptscriptstyle T} }}
\newcommand{\indep}{\perp\!\!\!\perp}
\newcommand{\nindep}{\perp\!\!\!\perp\!\!\!\!\!\!/\;\;}

\newcommand{\med}{{\rm med}}
\newcommand{\card}{{\rm card}}
\newcommand{\bs}{\boldsymbol}
% \newcommand{\do}{{\rm do}}
\newcommand{\Splus}{\textsc{S-Plus}\ }
%\newcommand{\R}{\texttt{R} }

% statistical notation

\def\rmi{{\rm i}}
\def\pr{{\rm Pr}}
\def\Pr{\pr}
\def\E{{\rm E}}
\def\Ev{{\rm Ev}}
\def\var{{\rm var}}
\def\avar{{\rm avar}}
\def\cov{{\rm cov}}  
\def\corr{{\rm corr}}  
\def\Estar{{\rm E^*\thinspace}}
\def\varstar{{\rm var^*\thinspace}}
\def\covstar{{\rm cov^*\thinspace}}  
\def\median{{\rm median}}  
\def\cum{{\rm cum}}
\def\IMSE{{\rm IMSE}}  
\def\AIC{{\rm AIC}}  
\def\BIC{{\rm BIC}}  
\def\NIC{{\rm NIC}}  
\def\AICc{{\rm AIC_c}}  
\def\CV{{\rm CV}}  
\def\GCV{{\rm GCV}}  
\def\IQR{{\rm IQR}}  
\def\MAD{{\rm MAD}}  
\def\Lik{{L}}
\def\logL{{\ell}}
\def\RLik{{RL}}
\def\logLp{{\ell_{\rm p}}}

\def\Dto{{\ {\buildrel D\over \longrightarrow}\ }}
\def\Pto{{\ {\buildrel P\over \longrightarrow}\ }}
\def\rto{{\ {\buildrel r\over \longrightarrow}\ }}
\def\2to{{\ {\buildrel 2\over \longrightarrow}\ }}
\def\Wto{{\ {\buildrel W\over \longrightarrow}\ }}
\def\psto{{\ {\buildrel \rm{p.s.}\over \longrightarrow}\ }}
\def\asto{{\ {\buildrel \rm{a.s.}\over \longrightarrow}\ }}
\def\iid{{\ {\buildrel \rm{iid}\over \sim}\ }}
\def\ind{{\ {\buildrel \rm{ind}\over \sim}\ }}
\def\dotsim{{\ {\buildrel \cdot\over \sim}\ }}
%\def\sim{{\ {\sim}\ }}
%\def\to{{\longrightarrow}}
\def\Deq{{\ {\buildrel D\over =}\ }}
\def\Eoneton{{$E_1,\ldots,E_n$}}
%\def\T1ton{{$T_1,\ldots,T_n$}}
\def\I1ton{{$I_1,\ldots,I_n$}}
%\def\U1ton{{$U_1,\ldots,U_n$}}
\def\X1ton{{$X_1,\ldots,X_n$}}
\def\Y1ton{{$Y_1,\ldots,Y_n$}}
\def\Z1ton{{$Z_1,\ldots,Z_n$}}
\def\R1ton{{$R_1,\ldots,R_n$}}
\def\e1ton{{$e_1,\ldots,e_n$}}
\def\t1ton{{$t_1,\ldots,t_n$}}
\def\x1ton{{$x_1,\ldots,x_n$}}
\def\y1ton{{$y_1,\ldots,y_n$}}
\def\z1ton{{$z_1,\ldots,z_n$}}
%\def\r1ton{{$r_1,\ldots,r_n$}}

% Journal abbreviations

\def\AAP{\emph{Advances in Applied Probability}}
\def\AnnProbab{\emph{Annals of Probability}}
\def\AISM{\emph{Annals of the Institute of Statistical Mathematics}}
\def\AMS{\emph{Annals of Mathematical Statistics}}
\def\ApplStatist{\emph{Applied Statistics}}
\def\AS{\emph{Annals of Statistics}}
\def\B{\emph{Bernoulli}}
\def\Bka{\emph{Biometrika}}
\def\CJS{\emph{Canadian Journal of Statistics}}
\def\CSDA{\emph{Computational Statistics \& Data Analysis}}
\def\Eca{\emph{Econometrica}}
\def\ISI{\emph{International Statistical Review}}
\def\ISR{\emph{International Statistical Review}}
\def\JAMA{\emph{Journal of the American Medical Association}}
\def\JAP{\emph{Journal of Applied Probability}}
\def\JASA{\emph{Journal of the American Statistical Association}}
\def\JBES{\emph{Journal of Business \& Economic Statistics}}
\def\JCGS{\emph{Journal of Computational and Graphical Statistics}}
\def\JSCS{\emph{Journal of Statistical Computation and Simulation}}
\def\JRSSA{\emph{Journal of the Royal Statistical Society series A}}
\def\JRSSB{\emph{Journal of the Royal Statistical Society series B}}
\def\JRSSD{\emph{The Statistician}}
\def\SJS{\emph{Scandinavian Journal of Statistics}}
\def\SPA{\emph{Stochastic Processes and their Applications}}
\def\SM{\emph{Survey Methodology}}
\def\SS{\emph{Statistical Science}}
\def\TAS{\emph{The American Statistician}}
\def\Tech{\emph{Technometrics}}
\def\ZW{\emph{Z. Wahrsch. v. geb.}}
\def\JC{\emph{Journal of Classification}}
\def\PNAS{\emph{Proceedings of the National Academy of Science}}

% utility macros

\def\np{{\newpage}}
\def\gap{{\vskip 0.3in}}
\def\etal{{\sl et al.}} 
\def\pound{{\it \$}}
\def\apriori{{\sl a priori }}
\def\examfoot{{\vfill\hfill{\bf Turn over}\eject}}
\def\newtransparency{{\newpage}}
\def\Section{{Section~}}
\def\Sections{{Sections~}}
\def\Pvalue{{P-value}}
\def\Pvalues{{P-values}}

\def\report#1{{\newpage\centerline{\bf #1}\smallskip}}

% odds and ends

\def\redbf#1{{\color{red}\bf #1}}%
\def\Defn{\redbf{Definition:\ }}%
\def\Thm#1{\redbf{Theorem #1:\ }}%
\def\Ex#1{\redbf{Example #1:\ }}%
\def\Note{\redbf{Note:\ }}%
\def\Exercise#1{\redbf{Exercise #1:\ }}%
\def\Ill{\redbf{Illustration:\ }}%
\def\endex{{\hfill\redbf{$\bullet$}\smallskip}}
\def\calP{{\mathcal{P}}}
\def\calS{{\mathcal{S}}}
\def\calI{{\mathcal{I}}}
\def\eme{{\`eme}}
\def\ere{{\`ere}}
%\def\picbox#1#2{{\centerline{\psfig{figure=#1,height=#2pc}}}}%
\def\picbox#1#2#3{{\centerline{\psfig{figure=#1,height=#2pc,angle=#3}}}}%
\def\tt#1{{\texttt{#1}}}
\def\Der#1{\textbf{D#1}}



==> teachingmacros.tex <==
% LaTeX macros

% Last modified: 25/12/08

%----------------------------------------------
%  Anthony Davison, Department of Mathematics,
%  EPFL, 1015 Lausanne, Switzerland
%  00 41 21 693 5502
%  Anthony.Davison@epfl.ch
%----------------------------------------------

% teaching macros

\def\redbf#1{{\color{red}\bf #1}}%
\def\red#1{{\color{red} #1}}%
\def\b#1{{\color{red}\bf #1}}%
\def\Defn{\redbf{Definition:\ }}%
\def\Thm#1{\redbf{Theorem #1:\ }}%
\def\Ex#1{\redbf{Example #1:\ }}%
\def\Note{\redbf{Note:\ }}%
\def\Exercise#1{\redbf{Exercise #1:\ }}%
\def\Ill{\redbf{Illustration:\ }}%
\def\endex{{\hfill\redbf{$\bullet$}\smallskip}}
\def\eme{{\`eme}}
\def\ere{{\`ere}}

\def\picbox#1#2#3{{\centerline{\psfig{figure=#1,height=#2pc,angle=#3}}}}%

\def\tt#1{{\texttt{#1}}}
\def\Der#1{\textbf{D#1}}

\newtheorem{defn}{Definition}
\newtheorem{alg}[defn]{Algorithm}
\newtheorem{theorem}[defn]{Theorem}
\newtheorem{lemma}[defn]{Lemma}
\newtheorem{example}[defn]{Example}
\newtheorem{cor}[defn]{Corollary}
\newtheorem{prop}[defn]{Proposition}

\def\ssim{{\ {\buildrel s\over \sim}\ }}
\def\vsim{{\ {\buildrel v\over \sim}\ }}

\def\halfback{{\vspace{-0.1in}}}
\def\back{{\vspace{-0.2in}}}
